Robust Federated Learning Against Adversarial Attacks for Speech Emotion Recognition

Due to the development of machine learning and speech processing, speech emotion recognition has been a popular research topic in recent years. However, the speech data cannot be protected when it is uploaded and processed on servers in the internet-of-things applications of speech emotion recognition. Furthermore, deep neural networks have proven to be vulnerable to human-indistinguishable adversarial perturbations. The adversarial attacks generated from the perturbations may result in deep neural networks wrongly predicting the emotional states. We propose a novel federated adversarial learning framework for protecting both data and deep neural networks. The proposed framework consists of i) federated learning for data privacy, and ii) adversarial training at the training stage and randomisation at the testing stage for model robustness. The experiments show that our proposed framework can effectively protect the speech data locally and improve the model robustness against a series of adversarial attacks.

==> README <==

August 26, 2015


IEEEtran is a LaTeX class for authors of the Institute of Electrical and
Electronics Engineers (IEEE) transactions journals and conferences.
The latest version of the IEEEtran package can be found at CTAN:

http://www.ctan.org/pkg/ieeetran

as well as within IEEE's site:

http://www.ieee.org/


This package contains the IEEE Computer Society subset of the full IEEEtran
package and is intended for use with IEEE Computer Society publications.
The included version of the IEEEtran_HOWTO.pdf has been specially formatted
in IEEE Computer Society (compsoc) journal mode.


For latest news, helpful tips, answers to frequently asked questions,
beta releases and other support, visit the IEEEtran home page at my
website:

http://www.michaelshell.org/tex/ieeetran/

Version 1.8b has a number of significant changes over the v1.8a release.
For a full history of changes, please read the file changelog.txt.
The most notable changes in this release include:

 1) Added new comsoc mode for the IEEE Communications Society.
    This mode (at present) only invokes the use of the newtxmath math fonts.
 
 2) Revised IEEEeqnarray column specifications to work with active " 
    (or other punctuation catcode changes) as with babel under the
    german or ngerman language modes. 
    Thanks to Stefan M. Moser for reporting this problem.

 3) Added \indexspace and other index related macros as newer versions of
    article.cls now do. These macros are needed to avoid an error when
    using the glossaries package.
    Thanks to Sebastian Nyberg for suggesting this change.

 4) Fixed odd/even page header font bug under compsoc mode and
    other page style code improvements.
    Thanks to Marco Paolieri for reporting this problem.

 5) Added hooks to allow for easy control of spacing above title.

 6) Added the \IEEEnoauxwrite command.
    Thanks to Sudarshan Mukherjee for suggesting this feature.


NOTE: Take care not to confuse the "comsoc" and "compsoc" class
options/modes as they are very different:

comsoc  ==> IEEE Communications Society
compsoc ==> IEEE Computer Society

The comsoc mode requires that an acceptable Times math font be available on
the LaTeX system. This requirement will be enforced by IEEEtran in comsoc
mode. Either the freely available newtxmath font by Michael Sharpe
http://www.ctan.org/pkg/newtx
(version 1.451, July 28, 2015 or later is recommended)
or the commercial MathTime font (e.g., mtpro2.sty) is acceptable.
See Section II-D (2.4) "Class Options - comsoc, compsoc, transmag" of
the IEEEtran HOWTO for more details.


Best wishes for all your publication endeavors,

Michael Shell
http://www.michaelshell.org/


********************************** Files **********************************

README                 - This file.

IEEEtran.cls           - The IEEEtran LaTeX class file.

changelog.txt          - The revision history.

IEEEtran_HOWTO.pdf     - The IEEEtran LaTeX class user manual.

bare_conf_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         conference papers.

bare_jrnl_compsoc.tex  - A bare bones starter file for IEEE Computer Society
                         journal papers.

bare_adv.tex           - A bare bones starter file showing advanced
                         techniques such as conditional compilation,
                         hyperlinks, PDF thumbnails, etc. The illustrated
                         format is for a IEEE Computer Society journal paper.

***************************************************************************
Legal Notice:
This code is offered as-is without any warranty either expressed or
implied; without even the implied warranty of MERCHANTABILITY or
FITNESS FOR A PARTICULAR PURPOSE! 
User assumes all risk.
In no event shall the IEEE or any contributor to this code be liable for
any damages or losses, including, but not limited to, incidental,
consequential, or any other damages, resulting from the use or misuse
of any information contained here.

All comments are the opinions of their respective authors and are not
necessarily endorsed by the IEEE.

This work is distributed under the LaTeX Project Public License (LPPL)
( http://www.latex-project.org/ ) version 1.3, and may be freely used,
distributed and modified. A copy of the LPPL, version 1.3, is included
in the base LaTeX documentation of all distributions of LaTeX released
2003/12/01 or later.
Retain all contribution notices and credits.
** Modified files should be clearly indicated as such, including  **
** renaming them and changing author support contact information. **

File list of work: IEEEtran.cls, IEEEtran_HOWTO.pdf, bare_adv.tex,
                   bare_conf_compsoc.tex, bare_jrnl_compsoc.tex.
***************************************************************************


==> sections/experiments_and_results_backup.tex <==
\section{Experiments and Results} \label{sec:experiments_and_results}
\subsection{Dataset} \label{sec:dataset}
\comment{
To validate the proposed framework, two emotional speech databases are used in our experiments. The details of the two databases are introduced as follows. }
\comment{
\begin{table}[ht]
\centering
\caption{Emotion distribution of the applied IEMOCAP dataset.
%\comZR{all columes have different widths, and should the numbers be aligned right?}\comYC{Table I is aligned central?}\comZR{oh, they are different. Or you could add space before the numbers XXX, because the numbers should align at the same colume from right to left}\comZR{OK, this one is done!}
}
\begin{tabular}{P{1cm}|P{1cm}|P{1cm}|P{1cm}|P{1cm}|P{1cm}}
\toprule
\# & Anger & Happiness & Neutral & Sadness & $\sum$ \\ \hline
Train & \ \ 881 & 1,301 & 1,392 & \ \ 851 & 4,425\\ \hline
Test & \ \ 222 & \ \ 335 & \ \ 316 & \ \ 233  & 1,106\\ \hline
$\sum$ & 1,103 & 1,636 & 1,708 & 1,084& 5,531\\ \bottomrule
\end{tabular}
\label{tab:iemocap}
\end{table}}

\begin{table}[ht]
\centering
\caption{Emotion distribution of the applied DEMoS dataset.
%\comZR{the same issue as before. shall we rotate the table to save space?}\comZR{Done! I have rotated it.}
}
\begin{tabular}{P{1cm}|P{1cm}|P{1cm}|P{1cm}}
\toprule
\# & Train & Test & $\sum$ \\
\hline
Anger &1,155 &\ \ 322 &1,477 \\
\hline
Disgust &1,354 &\ \ 324 &1,678 \\
\hline
Fear &\ \ 927 &\ \ 229 &1,156 \\
\hline
Guilt &\ \ 898 &\ \ 231 &1,129 \\
\hline
Happiness &1,127 &\ \ 268 &1,395 \\
\hline
Sadness &1,228 &\ \ 302 &1,530 \\
\hline
Surprise &\ \ 802 &\ \ 198 &1,000 \\
\hline
$\sum$ &7,491 &1,874 &9,365 \\
\bottomrule
\end{tabular}
\label{tab:demos}
\end{table}

% \begin{table*}[ht]
% \centering
% \caption{Emotion distribution of the applied DEMoS dataset.\comZR{the same issue as before. shall we rotate the table to save space?}}
% \begin{tabular}{c|c|c|c|c|c|c|c|c}
% \hline
% \# & Anger & Disgust & Fear & Guilt & Happiness & Sadness & Surprise & $\sum$ \\ \hline
% Train & 1155 & 1354 & 927 & 898 & 1127 & 1228 & 802 & 7491 \\ \hline
% Test & 322 & 324 & 229 & 231 & 268 & 302 & 198 & 1874 \\ \hline
% $\sum$ & 1477 & 1678 & 1156 & 1129 & 1395 & 1530 & 1000 & 9365 \\ \hline
% \end{tabular}
% \label{tab:demos}
% \end{table*}

\comment{
\subsubsection{IEMOCAP}
The Interactive Emotional dyadic MOtion CAPture (IEMOCAP) database~\cite{busso2008iemocap} consists of approximately 12 hours of audio-visual recordings. During recording, five pairs of actors (a female and a male) performed selected emotional scripts and also communicated with each other in scenarios designed to elicit specific types of emotions. The recordings were then segmented into utterances. Furthermore, the utterances were annotated into the emotional states, \ie \emph{anger}, \emph{disgust}, \emph{excited state}, \emph{fear}, \emph{frustration}, \emph{happiness}, \emph{neutral state}, \emph{sadness}, and \emph{surprise}. 

All audio recordings are sampled with $16$\,kHz in our experiments. Considering the class imbalance nature, we only consider four classes, including \emph{anger}, \emph{happiness }, \emph{neutral state}, \emph{sadness}. Please note that in order to be consistent with prior research~\cite{Chatziagapi2019, ISSA2020101894, 8817913} and try to maintain class balance, we include \emph{excited state} in \emph{happiness}. In this way, there are in total of $5,531$ samples from the IEMOCAP datasets are aplied in this work (average duration: $4.55$\,seconds $\pm$ standard deviation: $3.23$\,seconds). 

Since federated learning aims to long-termly perform on each speaker's data, we divide the database into a training set and a test set with the speaker-dependent strategy rather than the classic speaker-independent one. Each actor's speech is divided into an 80\,\% training set and a 20\,\% test set, each of which composes the global training set and test set, respectively. The emotion distribution is described in Table~\ref{tab:iemocap}.}


% \subsubsection{DEMoS}
The Database of Elicited Mood in Speech (DEMoS)~\cite{parada2019demos} is an Italian emotional speech corpus of $7.7$ hours of audio recordings. DEMoS was collected from $68$ speakers (23 females and 45 males) when the speakers' emotion were induced by an arousal-valence progression. In total, $9,365$ emotional and $332$ neutral speech samples were recorded. As the neutral state is a minority class, it is not considered in our experiment. Therefore, we employ the $9,365$ emotional speech samples (average duration: $2.86$ seconds $\pm$ standard deviation: $1.26$\,seconds) annotated into seven classes, including \textit{anger}, \textit{disgust}, \textit{fear}, \textit{guilt}, \textit{happiness}, \textit{sadness}, and \textit{surprise}. 

All audio recordings are sampled with $16$\,kHz in our experiment.  Since federated learning aims to long-termly perform on each speaker's data, we divide the database into a training set and a test set with the speaker-dependent strategy rather than the classic speaker-independent one. Each actor's speech is divided into an 80\,\% training set and a 20\,\% test set, each of which composes the global training set and test set, respectively. The emotion distribution is described in Table~\ref{tab:demos}
\comment{Due to the federated learning paradigm, DEMoS is speaker-dependently split into a training set and a test set. The division procedure is the same as that of IEMOCAP, leading to the emotion distribution in Table~\ref{tab:demos}.}



\subsection{Experimental Setup}
% @Yi, Sofiane
% \comZR{
% Yi: decided if to add a table with hyperparameters; 
% model structures $->$ appendix.
% - mention we tried several models and found resnet is better than others on iemocap for centralised learning.
% Zhao: check if we can add appendix (yes - appendix section has been added after conclusion)
% }

\textbf{Log Mel Spectrograms Extraction:}
As for DEMoS, we unify the audio sample length as the maximum one as 5.884\,seconds, which means shorter audio samples will be self-repeated. \comment{Similarly, we unify the length of each audio sample in the IEMOCAP as 5.984\,seconds by simply cutting the signals after the 5.984\,seconds from the original waves and shorter ones are self-repeated until the 5.984\,seconds. To note that 5.984\,seconds is around the $80^{th}$ percentile of all IEMOCAP audio lengths.} We set the sliding window as 512 time frames, overlap as 256 time frames, and Mel bins as 64 for the log Mel spectrograms extraction. In this way, the generated log Mel spectrograms share the dimension of (373, 64), where 373 is the dimension along the time steps, and 64 is the Mel frequencies. 

\textbf{Model's Architecture:}
VGG and VGG-like architectures have been widely applied in classifying spectrogram images in many audio tasks and shown their good performances~\cite{10.3389/fdgth.2021.799067, 9054087}. Therefore, in this work, we trained VGG-15 models in the federated setting.

As shown in Figure~\ref{fig:models}, the architecture of VGG-15 consists of five convolutional blocks with the output channel numbers of 64, 128, 256, 512, and 512, each of which is followed a local max pooling layer with the kernel size of $(2,2)$. Each convolutional layer is followed by a batch normalisation later and a `relu' activation function~\cite{relu} to stabilise and accelerate the training process~\cite{Ren2018AttentionbasedCN}. Before the final two fully connected layers for the final classification, a global average pooling layer is applied.
% \comZR{ResNet was not mentioned}


\textbf{Adversarial Federated Training:}
The maximal iteration for the optimisation procedure in DeepFool is set as 5, since the study~\cite{moosavi2016deepfool} stated that DeepFool empirically converges less than 3 iterations for a perturbation to fool the classifier. For better comparison, we also set the max iteration for PGD as 5. Moreover, we set the norm of the generated perturbation for FGSM, PGD, and DeepFool as $l_{\infty}$, $l_{\infty}$, and $l_{2}$, respectively as default. The $\epsilon$ in Equation~(\ref{eq:FGSM}), $\eta$ in Equation~(\ref{eq:PGD}), and $\zeta$ in Equation~(\ref{eq:DeepFool}) are set as 0.05, 0.05, 0.02, respectively. Moreover, the adversarial attack settings for adversarial training and testing are the same. Some generated adversarial examples are visualised in Fig.~\ref{fig:deepfool}. It can be seen that DeepFool trends to generate more imperceptible attacks to fool the classifier, compared with FGSM and PGD.

We set the $\alpha$ in Equation~(\ref{eq:vanilla_advTrain}) as 0.5, which means half original samples $X_{i}$ from client $\mathcal{F}_{i}$ are randomly selected from $\mathcal{D}_{i}$ to generate the corresponding adversarial examples $X_{advi}$ along with the remaining half original samples to train the model to have a fair comparison with the general federated learnt models.

The batch size for training is set to 8 considering the limitation of memory, whereas for validation and testing is 1 to maximise the ability of randomisation. 
The `Adam' optimiser is applied with an initial learning rate as 0.001 and the cosine decay policy to stabilise the training process.


For the FL implementation, We used our framework which is using Flower FL framework, where we adapted Docker to containerise our FL clients and FL server. That means that each FL client is running inside a Docker container and communicates with the FL server container. Once the FL training is complete, a model with the aggregated weights of the last round is saved for evaluation.gmail

\textbf{Randomisation:}
Original dimension of the generated log Mel spectrogram is (373, 64, 1). In Equation~(\ref{eq:randomisation}), the $W'$ is randomly chosen in [373, 380), and $H'$ is randomly chosen in [64, 66). After the resizing, we applied the random padding on the boundaries of the log Mel spectrogram by the value 0.5 and after the padding, the final $(W'', H'', 1)$ dimension is (380, 66, 1). We fine-tuned the hyper-parameters (\ie range that $W'$ are $H'$ chosen from, and values of $W''$ and $H''$ ) of the randomisation based on the set-aside validation dataset. 

\textbf{Reproducibility:}
For the implementation of the experiments, we used Flower framework \footnote{https://flower.dev}, which is an open source framework to run Federated Learning. For generating the adversarial data, Adversarial Robustness Toolbox (ART) \cite{art2018} open-source library was used, that contains the DeepFool, FGSM and PGD white-box attacks. 
From the hardware side, the experiments are conducted on Nvidia DGX machine \footnote{https://www.nvidia.com/en-us/data-center/dgx-station-a100}, which has 8x NVIDIA A100, with 8 GPUs with a total of 320GB GPU memory, an AMD 7742, 64 cores 2.25 GHz CPU \& 512GB of RAM. DGX is a powerful machine that allowed us to run the FL experiments at scale by running 68 FL client Docker containers and an FL server container simultaneously. 
%Our source code is available under (link)

\comment{
\begin{figure}
    \centering
    \includegraphics[width=.35\textwidth]{sections/figures/models_tac.pdf}
    \caption{Models architectures. (a) VGG-15 for the DEMoS dataset and (b.1) ResNet-6 for the IEMOCAP dataset. Specifically, building blocks are in square brackets with numbers of stacked blocks and every convolutional layer in the square brackets is followed by a batch normalisation layer. Please note that brackets in (b.1) contain the shortcut connection as shown in (b.2).}
    \label{fig:models}
\end{figure}}


\begin{figure}
    \centering
    \includegraphics[width=.20\textwidth]{sections/figures/models_tac3.pdf}
    \caption{VGG-15 architectures. Specifically, building blocks are in square brackets with numbers of stacked blocks and every convolutional layer in the square brackets is followed by a batch normalisation layer.}
    \label{fig:models}
\end{figure}


\subsection{Evaluation Metrics} 
\comment{
Accuracy, same as weighted average recall, is utilised in this work mainly for monitoring the federated models performance on the original test sample with the increasing rounds.} 

Compared with accuracy (\ie weighted average recall), Unweighted Average Recall (UAR) can better evaluate models' classification performance on imbalanced datasets~\cite{uar1}. UAR is used for further evaluate the converged federated models' performance on randomised data, adversarial examples, and randomised adversarial examples. 

\comment{Confidence Interval (CI) is applied in this work to measure the significance of the models' improvement. \comZR{please comment it if we didn't use CI}}

\subsection{Experimental Results}
% @Sofiane, Yi: fill all results as tables


% \subsubsection{Comparison of Federated Defences}
% For each following experiments let's consider different metrics for evaluating the final model that we obtain from each of the experiment settings outlined below:
% -accuracy = unweighted average recall (UAR);
% -F1-score;
% -Confusion matrix; 
% -CI (confidence interval) values on the test set. 
% Note: as discussed previously, we want to have for each client, a training and testing set. Therefore, each of these metrics  can be computed for:
% -The local participant (how much does each participant gain from the final model on its own local test set. For instance, some participants might gain more from this federated learning process than others.)
% -Globally, through pooling this test data, and computing these scores globally.
%TODO clarify if the evaluation per client idea is deprecated, and only go for the global test data


% For each dataset:
% \begin{enumerate}
% \item Accuracy vs Number of Rounds with \& without attack types + without defence (e.g. Fig. 2 in FDA3 paper).
% \item Accuracy vs Number of Rounds with attack types + with defence (adversarial training) (e.g. Fig. 2 in FDA3 paper)
% \item Accuracy vs Number of Rounds with \& without attack types +  with defence (randomisation)
% \item Accuracy vs Number of Rounds with \& without attack types +  with defence (adversarial training + randomisation)

%\item Performance (with attack types) of adversarial training and randomisation on the test set (e.g. Fig. 4 in FDA paper)
%\item (Note: randomisation is a layer of the model with random seed) On the training set, one randomisation pattern or several together? We have to come up with exp using randomisation...where (is it possible to choose/fix from a subset of randomisation techniques, e.g., to only have 3/6 in play, cropping, resize, flip, rotate, etc?)?

%\comGP{So, in this instance we have the randomisation equivalent of training against one white-box attack, and then evaluating against images perturbed based on attacks chosen uniformly across our available white-box attacks, just in this case it is for randomisation attacks. E.g., trained using a certain type of cropping, then in testing the image can be cropped, resized, etc. Potentially all at the same time, cropping, flipping, resizing...?}  




% ok. perhaps under Section \ref{sec:dataset} we should also clearly define these train/test splits. In the last meeting we discussed that there will be a train/test split on each client (i.e., each client has a testing set that it can use for local evaluation. and then we can aggregate the results to get a measure of the overall performance. Let's call that scenario A. 
% What you are describing we could call scenario B., where (if I understand correctly), we set a few clients to one side during training, and then add them later on. So essentially we have test clients?}

% \comGP{> "It may be initially bad, but will become better during fine-tuning. Yes, defence is also expected." 
% What is meant by fine-tuning in this setting? Are incorporating the test-clients in the training process, and the aim is to see how fast they can adapt?  
% }
% \comZR{You remind me this point, Greg, thanks. Yes, it would be initially bad and become better by fine-tuning. I wanted this to be compared with SOTA. But in federated learning, it's not possible to show the performance on the whole test set because we will do fine-tuning on part of the test set. So now I don't suggest this scenario-B, as well as SOTA comparison. 
% For SOTA supervised learning settings, the models mostly verified on all data of new subjects (clients). We cannot have the same test with SOTA methods.}
% \comMF{I try to summarize otherwise we have to read the entire comment each time :) : We have Scenario A where each client will have test sets and then we aggregate all performance results. This scenario could be simpler: we get from each client a test set data and the we aggregate the local test data set in a global test set. If we do so, it will be possible to use the same test set with SOTA}

% \item Best settings: Accuracy vs Percentage of Clients (e.g. Fig. 7 in FDA3 paper)

%\item \comZR{Probably random strategy to mix multiple kinds of attacks} \comGP{Yep, like this. In particular as it can later serve as a baseline (random policy) for our planned NeurIPS topic :-)... good to implement and gather results for this already.}
%\comMF{Really nice, but I will leave as priority 2 due to time constraints}
% \end{enumerate}


\begin{figure}
    \centering
    \includegraphics[width=.5\textwidth]{sections/figures/demos_68_uar.jpg}
    \caption{Performance comparison on test data between general federated learnt model, and federated adversarial trained models with DeepFool, FGSM and PGD algorithms. The models are evaluated at each $10^{th}$ round. Specifically, in the legends, `Nature' represents the general federated learnt model; `AdvTrain' means the adversarial training; `Attk.' means adversarial attack.}
    \label{fig:68_models}
\end{figure}

Fig.~\ref{fig:68_models} illustrates the UAR score of the trained FL models, comparing the general federated learnt model and the federated adversarial trained models with PGD, FGSM  and DeepFool, respectively. The models are evaluated on the real test data after each 10 rounds.
The four mentioned models converge to around 90\% UAR score with diverse convergence time. We can see that, the federated adversarial training with the three algorithms share similar convergence speed with the nature model, where all models herein converge after 150 rounds. Therefore, we conduct further test for the above models after 150 rounds until the final 300 rounds, every 10 rounds.

%TODO include the graph for centralised Demos, and interpret it

\comment{
\comYC{In Table~\ref{tab:res-rand-1} and Table~\ref{tab:res-rand-2}, we exhibit the performance of general federated learnt VGG model (180 rounds, 68 clients, 1 epoch).  The epsilon for FGSM, PGD, and DeepFool is 0.002, 0.002, 0.02 respectively. The batch size and max iteration for PGD and DeepFool are 32 and 50. In Table~\ref{tab:res-rand-2}, the epsilon for FGSM, PGD, and DeepFool is 0.005, 0.005, 0.02 respectively. The batch size and max iteration for PGD and DeepFool are 32 and 50. }}


\comment{
\begin{table}[]
    \centering
    \caption{The performance (top-1 classification accuracy [\%]) on the test dataset of original federated learnt model with different adversarial attack methods. `Org' means original test dataset; `Adv' indicates the adversarial examples generated based on the original test dataset; `Rand Org' refers to randomised original test dataset; `Rand Adv' is the randomised adversarial examples.}
    \begin{tabular}{l|l|l|l|l}
    \hline
    Attacks & Org & Adv & Rand Org & Rand Adv \\ \hline
    FGSM & 86.86 & 69.66 & 85.79 & 78.31 \\ \hline
    PGD & 86.86 & 66.67 & 86.25 & 77.71 \\ \hline
    DeepFool & 86.86 & 6.20 & 85.90 & 74.32 \\ \hline
    \end{tabular}
    \label{tab:res-rand-1}
\end{table}
}

\comment{
\begin{table}[]
    \centering
    \caption{The performance (top-1 classification accuracy [\%]) on the test dataset of original federated learnt model (VGG, 180 rounds, 68 clients, 1 epoch) with different adversarial attack methods.}
    \begin{tabular}{l|l|l|l|l}
    \hline
    Attacks & Org & Adv & Rand Org & Rand Adv \\ \hline
    FGSM & 86.86 & 24.04 & 86.08 & 51.42 \\ \hline
    PGD & 86.86 & 16.56 & 85.90 & 48.43 \\ \hline
    DeepFool & 86.86 & \red 6.20 & 85.61 & \red 74.04 \\ \hline
    \end{tabular}
    \label{tab:res-rand-2}
\end{table}
}
\comment{
\comYC{Since all adversarial trained federated models have the results of 220 rounds, 68 clients, and 1 epoch, in Table~\ref{tab:res-rand-3}, we compare three different models trained with FGSM, PGD, and DeepFool adversarial generated exmpales. \textbf{Considering the memory issue and time constrains, the batch size and max iteration for PGD and DeepFool are 1 and 5 for training and testing. \red We need to make the batch size, max iteration (especially) consistent for training and testing?! The number of rounds for federated training V.S. the number of rounds for adversarial federated training?!}}}

\comment{
\begin{table}[]
    \centering
    \caption{The performance (top-1 classification accuracy [\%]) on the test dataset of adversarial trained federated models under theirs corresponding attack methods. `Org' means original test dataset; `Adv' indicates the adversarial examples generated based on the original test dataset; `Rand Org' refers to randomised original test dataset; `Rand Adv' is the randomised adversarial examples.}
    \begin{adjustbox}{width=0.98\columnwidth,center}
    \begin{tabular}{l|l|l|l|l}
    \hline
    models & Org & Adv & Rand Org & Rand Adv \\ \hline
    FGSM-adversarial & 85.68 & 45.19 & 84.26 & 68.23 \\ \hline
    PGD-adversarial & 89.21 & 48.72 & 87.78 & 64.42 \\ \hline
    DeepFool-adversarial & 86.11 & \red 5.34 & 84.86 & \red 54.38 \\ \hline
    \end{tabular}
    \label{tab:res-rand-3}
    \end{adjustbox}
\end{table}
}


\comment{
\begin{table}[]
    \centering
    \caption{The performance (UAR [\%]) of the classic federated learning when it is deceived by adversarial attacks. (will be a line chart)}
    \begin{tabular}{c|c|ccc}
    \toprule
         \# Epoch & wo/attack & \multicolumn{3}{c}{w/ attack}   \\
         & & FGSM & PGD & DeepFool \\
        \hline
        &\\
    \bottomrule
    \end{tabular}
    \label{tab:result_no_defence}
\end{table}}

\comment{
\begin{table*}[]
    \centering
    \caption{The performance (UAR [\%]) of federated learning with adversarial training randomisation, and both, when it is deceived by adversarial attacks. (will be a line chart)}
    \begin{tabular}{c|ccc|ccc|ccc}
    \toprule
    & \multicolumn{3}{c|}{adversarial training} & \multicolumn{3}{c|}{randomisation} & \multicolumn{3}{c}{adv. training + randomisation}\\
         \# Epoch & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool\\
        \hline
        &\\
    \bottomrule
    \end{tabular}
    \label{tab:result_at}
\end{table*}}


\comment{
\begin{table*}[]
    \centering
    \caption{The performance (accuracy [\%]) of federated learning with adversarial training randomisation, and both, when it is deceived by adversarial attacks('-' means no attack) on the test set. (will be a histogram figure)}
    \begin{tabular}{c|cccc|cccc|cccc|cccc}
    \toprule
    & \multicolumn{4}{c|}{federated training} &
    \multicolumn{4}{c|}{adversarial training} &
    \multicolumn{4}{c|}{randomisation} & \multicolumn{4}{c}{adv. training + randomisation}\\
         \# Round  & - & FGSM & PGD & DeepFool & - & FGSM & PGD & DeepFool & - & FGSM & PGD & DeepFool & - & FGSM & PGD & DeepFool\\
        \hline
        160  & & & &  &  &  &  &  &  &  &  &  & & & &  \\
    \bottomrule
    \end{tabular}
    \label{tab:result_at}
\end{table*}
}

\comment{
\begin{figure*}
    \centering
    \includegraphics[width=.99\textwidth]{sections/figures/tab_res_demos.pdf}
    \caption{}
    \label{fig:res_tab}
\end{figure*}}



\begin{figure*}
     \centering
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{sections/figures/demos/demos_1.png}
         \caption{}
         \label{fig:demos1}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{sections/figures/demos/demos_2.png}
         \caption{}
         \label{fig:demos2}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{sections/figures/demos/demos_3.png}
         \caption{}
         \label{fig:demos3}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.46\textwidth}
         \centering
         \includegraphics[width=\textwidth]{sections/figures/demos/demos_4.png}
         \caption{}
         \label{fig:demos4}
     \end{subfigure}
        \caption{Performance on DEMoS every 10 rounds until 300 rounds. (a) shows the results of models tested on the original test dataset; (b) depicts the results on the randomised test dataset; (c) shows the results on the adversarial samples; (d) displays the performances on the randomised adversarial samples. Specifically, in the legends, `Nature' represents the federated learnt model; `AdvTrain' means the adversarial training; `Attk.' means adversarial attack.}
        \label{fig:demos_res_tab}
\end{figure*}


\begin{figure}
     \centering
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{sections/figures/demos/matrix_fgsm_2.png}
         \caption{}
         \label{fig:cf_fgsm}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{sections/figures/demos/matrix_pgd_2.png}
         \caption{}
         \label{fig:cf_pgd}
     \end{subfigure}
     \hfill
     \begin{subfigure}[b]{0.45\textwidth}
         \centering
         \includegraphics[width=\textwidth]{sections/figures/demos/matrix_deepfool_2.png}
         \caption{}
         \label{fig:cf_deepfool}
     \end{subfigure}
        \caption{Confusion matrices for adversarial training models under adversarial attacks after $300$ rounds on the DEMoS test dataset. `gui': Guilt, `dis': Disgust, `hap': Happiness, `fea': Fear, `ang': Anger, `sur': Surprise, `sad': Sadness.}
        \label{fig:cf_demos}
\end{figure}





%%%%%%%%% Yi Chang Added, Jan 23, 2022 %%%%%%%%%%%%
\comment{
\begin{table*}[]
    \centering
    \caption{The performance (UAR [\%]) of federated learnt general models on the test dataset, when it is deceived by adversarial attacks.}
    \begin{tabular}{ccc|ccc|ccc}
    \hline
    \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{Adversarial Attack} & \multicolumn{3}{c}{randomised Adversarial Attack} \\
    \multicolumn{1}{c|}{\# Round} & \multicolumn{1}{c|}{Original} & randomisation & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool \\ \hline
    \multicolumn{1}{c|}{150} & \multicolumn{1}{c|}{92.18} & 89.03 & 14.45 & 7.89 & 4.01 & 37.73 & 33.48 & 69.63 \\
    \multicolumn{1}{c|}{160} & \multicolumn{1}{c|}{91.91} & 88.93 & 16.46 & 9.36 & 4.51 & 40.71 & 35.73 & 71.48 \\
    \multicolumn{1}{c|}{170} & \multicolumn{1}{c|}{91.68} & 88.84 & 17.24 & 9.72 & 4.84 & 40.36 & 35.88 & 72.77 \\
    \multicolumn{1}{c|}{180} & \multicolumn{1}{c|}{92.61} & 89.55 & 17.54 & 9.33 & 4.16 & 43.19 & 37.84 & 72.48 \\
    \multicolumn{1}{c|}{190} & \multicolumn{1}{c|}{93.37} & 90.86 & 14.24 & 7.59 & 2.61 & 41.83 & 36.34 & 74.00 \\
    \multicolumn{1}{c|}{200} & \multicolumn{1}{c|}{92.14} & 89.31 & 17.53 & 9.59 & 3.73 & 42.48 & 38.44 & 71.15 \\
    \multicolumn{1}{c|}{210} & \multicolumn{1}{c|}{92.61} & 88.35 & 17.27 & 9.04 & 3.96 & 39.59 & 34.95 & 65.18 \\
    \multicolumn{1}{c|}{220} & \multicolumn{1}{c|}{93.43} & 91.37 & 17.72 & 9.21 & 3.23 & 44.10 & 38.84 & 71.23 \\
    \multicolumn{1}{c|}{230} & \multicolumn{1}{c|}{93.26} & 91.32 & 16.33 & 8.70 & 2.78 & 43.93 & 38.05 & 71.13 \\
    \multicolumn{1}{c|}{240} & \multicolumn{1}{c|}{93.14} & 91.56 & 18.05 & 8.87 & 3.23 & 44.90 & 38.91 & 73.30 \\
    \multicolumn{1}{c|}{250} & \multicolumn{1}{c|}{93.73} & 91.07 & 19.73 & 10.12 & 3.41 & 44.09 & 38.38 & 67.97 \\
    \multicolumn{1}{c|}{260} & \multicolumn{1}{c|}{93.10} & 91.46 & 19.42 & 9.78 & 3.77 & 45.16 & 38.69 & 70.31 \\
    \multicolumn{1}{c|}{270} & \multicolumn{1}{c|}{93.02} & 91.05 & 17.78 & 8.89 & 3.21 & 42.79 & 36.98 & 72.29 \\
    \multicolumn{1}{c|}{280} & \multicolumn{1}{c|}{93.74} & 92.10 & 20.87 & 10.37 & 3.14 & 47.54 & 41.49 & 74.09 \\
    \multicolumn{1}{c|}{290} & \multicolumn{1}{c|}{93.51} & 92.26 & 20.13 & 9.70 & 3.15 & 47.10 & 40.72 & 72.68 \\
    \multicolumn{1}{c|}{300} & \multicolumn{1}{c|}{94.08} & 92.75 & 20.82 & 9.96 & 2.96 & 47.91 & 41.55 & 71.34 \\ \hline
    \end{tabular}
    \label{tab:result_fl}
\end{table*}}


\begin{table}[h]
\caption{The performance (UAR [\%]) of nature and adversarial federated learnt models after 300 rounds on the test dataset, when it is deceived by adversarial attacks. The type of adversarial attack is consistent with the one for generating the adversarial examples for adversarial training.}
\scalebox{0.9}{\begin{tabular}{c|c|rrrr}
\hline
Models & Test data & \multicolumn{4}{c}{Attacks} \\ \hline
\multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{No} & \multicolumn{1}{c|}{FGSM} & \multicolumn{1}{c|}{PGD} & \multicolumn{1}{c}{DeepFool} \\ \hline
\multirow{4}{*}{Nature} & Original & \multicolumn{1}{r|}{94.08} & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{-} & - \\ \cline{2-6} 
 & Randomised & \multicolumn{1}{r|}{92.75} & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{-} & - \\ \cline{2-6} 
 & Adversarial & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{20.82} & \multicolumn{1}{r|}{9.96} & 2.96 \\ \cline{2-6} 
 & Randomised adversarial & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{47.91} & \multicolumn{1}{r|}{41.55} & 71.34 \\ \hline
\multirow{4}{*}{\begin{tabular}[c]{@{}c@{}}Adversarial\\ federated \\ learnt\end{tabular}} & Original & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{95.99} & \multicolumn{1}{r|}{95.40} & 95.16 \\ \cline{2-6} 
 & Randomised & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{95.32} & \multicolumn{1}{r|}{95.10} & 94.56 \\ \cline{2-6} 
 & Adversarial & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{89.72} & \multicolumn{1}{r|}{87.31} & 1.98 \\ \cline{2-6} 
 & Randomised adversarial & \multicolumn{1}{r|}{-} & \multicolumn{1}{r|}{90.15} & \multicolumn{1}{r|}{89.20} & 72.32 \\ \hline
\end{tabular}}
\label{tab:result_fl}
\end{table}


% \begin{table*}[h]
%     \centering
%     \caption{The performance (UAR [\%]) of nature model on the test dataset, when it is deceived by adversarial attacks.}
%     \begin{tabular}{ccc|ccc|ccc}
%     \hline
%     \multicolumn{3}{c|}{} & \multicolumn{3}{c|}{Adversarial Attack} & \multicolumn{3}{c}{Randomised Adversarial Attack} \\
%     \multicolumn{1}{c|}{\# Round} & \multicolumn{1}{c|}{Original} & Randomisation & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool \\ \hline
%     \multicolumn{1}{c|}{300} & \multicolumn{1}{c|}{94.08} & 92.75 & 20.82 & 9.96 & 2.96 & 47.91 & 41.55 & 71.34 \\ \hline
%     \end{tabular}
%     \label{tab:result_fl}
% \end{table*}

\comment{
\begin{table*}[]
    \centering
    \caption{The performance (UAR [\%]) of federated learnt adversarial models on the test dataset, when it is deceived by adversarial attacks. The adversarial attack is consistent with the attack applied in the adversarial training.}
    \begin{tabular}{c|ccc|ccc|ccc|ccc}
    \hline
     & \multicolumn{3}{c|}{Original} & \multicolumn{3}{c|}{Randomisation} & \multicolumn{3}{c}{Adversarial Attack} & \multicolumn{3}{c|}{Randomised Adversarial Attack} \\
    \# Round & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool \\ \hline
    150 & 93.95 & 92.57 & 93.57 & 92.91 & 91.22 & 92.65 & 80.10 & 77.39 & 2.81 & 80.72 & 78.70 & 59.96 \\
    160 & 94.77 & 92.30 & 94.28 & 93.65 & 91.56 & 93.10 & 86.41 & 77.52 & 2.41 & 86.69 & 80.66 & 64.87 \\
    170 & 95.12 & 93.08 & 94.27 & 93.82 & 91.66 & 93.20 & 86.30 & 78.80 & 2.53 & 86.63 & 80.32 & 61.02 \\
    180 & 95.47 & 94.48 & 94.32 & 94.28 & 93.42 & 93.27 & 85.66 & 82.67 & 2.85 & 86.11 & 84.80 & 60.57 \\
    190 & 94.59 & 94.58 & 94.98 & 93.24 & 93.73 & 93.65 & 84.35 & 82.73 & 2.20 & 85.24 & 84.70 & 63.66 \\
    200 & 95.19 & 95.14 & 95.06 & 94.23 & 93.99 & 93.91 & 87.16 & 84.43 & 2.16 & 87.60 & 85.23 & 69.10 \\
    210 & 95.19 & 94.73 & 94.70 & 94.30 & 93.89 & 93.17 & 86.78 & 84.94 & 2.43 & 87.88 & 85.15 & 61.10 \\
    220 & 95.64 & 95.14 & 94.94 & 94.95 & 94.24 & 93.83 & 88.88 & 84.90 & 2.34 & 88.91 & 85.37 & 65.59 \\
    230 & 95.91 & 95.36 & 94.72 & 94.45 & 94.36 & 94.10 & 87.55 & 85.49 & 2.47 & 87.49 & 86.44 & 73.07 \\
    240 & 95.94 & 95.14 & 95.55 & 95.07 & 94.45 & 94.83 & 88.23 & 85.37 & 1.62 & 88.72 & 87.23 & 71.05 \\
    250 & 95.59 & 95.27 & 95.63 & 94.94 & 94.15 & 94.48 & 89.12 & 83.20 & 1.79 & 88.69 & 85.07 & 62.58 \\
    260 & 95.77 & 95.22 & 95.70 & 94.98 & 94.31 & 94.71 & 89.52 & 86.79 & 1.93 & 88.96 & 88.25 & 67.72 \\
    270 & 95.44 & 96.02 & 95.31 & 94.82 & 95.02 & 94.51 & 89.25 & 87.01 & 1.73 & 89.34 & 87.73 & 69.95 \\
    280 & 95.72 & 95.49 & 96.09 & 95.46 & 94.75 & 95.04 & 89.50 & 85.42 & 1.40 & 89.60 & 86.49 & 63.01 \\
    290 & 95.47 & 95.72 & 95.43 & 95.03 & 94.78 & 94.79 & 89.82 & 87.26 & 1.86 & 89.81 & 87.93 & 67.07 \\
    300 & 95.99 & 95.40 & 95.16 & 95.32 & 95.10 & 94.56 & 89.72 & 87.31 & 1.98 & 90.15 & 89.20 & 72.32 \\ \hline
    \end{tabular}
    \label{tab:result_adv}
\end{table*}}

% \begin{table*}[h]
%     \centering
%     \caption{The performance (UAR [\%]) of adversarial federated learnt models on the test dataset, when it is deceived by adversarial attacks. The adversarial attack is consistent with the attack applied in the adversarial training.}
%     \begin{tabular}{c|ccc|ccc|ccc|ccc}
%     \hline
%      & \multicolumn{3}{c|}{Original} & \multicolumn{3}{c|}{Randomisation} & \multicolumn{3}{c}{Adversarial Attack} & \multicolumn{3}{c}{Randomised Adversarial Attack} \\
%     \# Round & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool \\ \hline
%     300 & 95.99 & 95.40 & 95.16 & 95.32 & 95.10 & 94.56 & 89.72 & 87.31 & 1.98 & 90.15 & 89.20 & 72.32 \\ \hline
%     \end{tabular}
%     \label{tab:result_adv}
% \end{table*}

%\comZR{i donot suggest to keep table 5 and 6 as they are totally the same as fig 5. Could you please simplify them to the 300th round?} 
%\comYC{done}
% adversarial examples (\ie adversarial samples, ....)

From Fig.~\ref{fig:demos_res_tab}, there are mainly three major findings. Firstly, Fig.~\ref{fig:demos1} and Fig.~\ref{fig:demos2} show that adversarial learnt models perform better than nature models; the randomisation layer herein itself only hurts the model's performance by little. Secondly, from Fig.~\ref{fig:demos3}, we can see that our adversarial training strategy is successful, helping models fight against the adversarial attacks, besides DeepFool. Thirdly, by comparing Fig.~\ref{fig:demos3} and Fig.~\ref{fig:demos4}, randomisation can further helps mitigate the adversarial attack effects, especially for nature models under FGSM, PGD and DeepFool attacks and adversarial federated learnt models under DeepFool attacks. 
However, as for the adversarial federated learnt models under FGSM and PGD attacks, the absolute improvement is not obvious. It is because adversarial training is the key step in defending the models against the FGSM and PDG attacks under our settings, which have strong transferability. On the other hand,  DeepFool is more likely to over-fitted to the target models and thus randomisation can better help to destroy the structure of perturbations. 


From Table~\ref{tab:result_fl}, there are several observations. Firstly, no matter for the nature models and federated adversarial trained models, randomisation is successful in mitigate the adversarial attacks. When we apply randomisation onto the original test dataset, the performance only drops a little bit (usually less than absolute 1\,\% on UAR). When randomisation is applied on the generated adversarial examples, it improves the performance by a large amount. It is because randomisation probably destroys the specific adversarial perturbations pattern~\cite{xie2018mitigating}. Specifically, randomisation better helps the models fight against the DeepFool attack, improving the UAR from 2.96\,\% to 71.34\,\% ($p < 0.001$ in a one-tailed z-test) for nature model and from 1.98\,\% to 72.32\,\% for adversarial federated learnt model ($p < 0.001$ in a one-tailed z-test). Moreover, the UAR improvements for nature models under FGSM (from 20.82\,\% to 47.91\,\%) and PGD (9.96\,\% to 41.55\,\%) attacks are also significant ($p < 0.001$ in a one-tailed z-test). Secondly, with the adversarial training, models' performances under the FGSM (20.82\,\% to 89.72\,\%) and PGD (9.96\,\% to 87.31\,\%) attacks improve a lot ($p < 0.001$ in a one-tailed z-test), probably since single-step attacks (\eg FGSM) and PGD in this settings, they are more transferable and hard to get over-fitted to the parameters of  specific neural networks ~\cite{xie2018mitigating}.  However, it seems that the adversarial training doesn't help the models to mitigate the DeepFool adversarial effects. The reason is that DeepFool iterates until the generated attack samples successfully fools the classifier, in which process DeepFool is more likely to over-fitted to the specific models and has less transferability~\cite{xie2018mitigating}. 

The confusion matrices of adversarial federated learnt models performances on the randomised adversarial test dataset after 300 rounds can be referred to Figure~\ref{fig:cf_demos}. From Fig.~\ref{fig:cf_fgsm} and Fig.~\ref{fig:cf_pgd}, we can see that most test samples are labelled correctly. However, in Fig.~\ref{fig:cf_deepfool},  many samples are misclassified into Disgust emotion, especially the Fear emotion. This can be caused by the Similar acoustic characteristics among these negative feelings.

%%%%%%%%% Yi Chang Added, 23 Jan 2022 %%%%%%%%%%%%

\comment{
\begin{table*}[]
    \centering
    \caption{The performance (UAR [\%]) of federated learning with adversarial training randomisation, and both, when it is deceived by adversarial attacks during federated learning and on the test set. (will be a histogram figure)}
    \begin{tabular}{c|ccc|ccc|ccc}
    \toprule
    & \multicolumn{3}{c|}{training} & \multicolumn{3}{c}{test set} &\\
         \# Epoch & FGSM & PGD & DeepFool & FGSM & PGD & DeepFool \\
        \hline
        &\\
    \bottomrule
    \end{tabular}
    \label{tab:result_at}
\end{table*}
}



  
% \subsubsection{Comparison with SOTA}
% \comZR{list SOTA methods , compare , analysis
% Sofiane, (Zhao helps)}

% \begin{enumerate}
% \item A table compares our performance on the test set and SOTA performance
% \end{enumerate}

% \begin{table}[h]
% \begin{tabular}{c|c|l}
% \hline
% UAR {[}\%{]} & Attk. & Test \\ \hline
% Zhao \etal & FGSM & 86.7 \\ \hline
% Our federated model & FGSM & 90.15 \\ \hline
% \end{tabular}
% \end{table}


%TODO discuss with Zhao
% Only in centralised mode (unless Sofiane can work some black magic ;-)... )
% -DeMoS: models in Zhao's iCAssp 2020 paper 
% -IEMOCAP: Zhao's work - find the best model
% - Apply all white box attacks
% \comGP{SOTA here is finding state-of-the-art methods that will serve as a baseline? If yes, then what approaches do we have in mind here?}
% \comZR{yes. we don't need to perform the SOTA approaches i think, just collecting the performance from other related papers. There are many SOTA methods. Most of them are supervised learning using deep learning models like CNNs, etc. }
% \comGP{I see, so essentially SOTA non-federated methods, that have been found to perform well in this domain? If we were not under time pressure, we might also want to federate these approaches, for an extensive comparison? Are we potentially running into the obvious review question here of: "if these approaches do so well, and are currently SOTA, then why did you not federate them?". I guess this is for a journal, so worst case scenario this might be a request if they chose to give us major revisions...}
% \comMF{Nice Greg that you found our next paper: adapting all SOTA to Fed. Lea., but out for the moment due to time constraints as you correctly pointed out}
% %ZR: I will check the SOTA test set and performance
% \comZR{same as 5), how about removing this part.}
% \comGP{Could we potentially compare the aggregated participant test set results from scenario A with the SOTA results? This should give us a fair comparison?} 
% \comGP{But indeed, I think this is a tactical question now. Also with respect to time (for the experiments that we have planned, we might also need to factor in some time for hyperparameter tuning, etc?). So perhaps better to have a few experiments less, but the ones that we do have in there, we do well? We could for now demonstrate awareness of these methods, by mentioning the plan to federate them in a future work section. Sofiane and I have a HiWi who could be tasked with adding them to the framework in the new year, in anticipation of the reviewers' responses. Perhaps: @Zhao: can you give us a list of these SOTA methods, and @Sofiane, @Yi, you guys could then consider if gathering implementations, and running experiments (potentially even federating one of them) is feasible within the remaining time?}
% \comMF{Agree for january, not for now. So, in summary we won't have SOTA comparison for the moment, right?}
% \comGP{Yeah, probably best to leave it for now I think, given the time constraints.}

%\subsection{Robustness Analysis}
%\comZR{remove}
% @Sofiane, Yi: fill all results as tables
%\begin{enumerate}
%    \item on the test set, accuracy vs new attack methods (a table) - show i) the initial attacked performance and ii) how many epochs are needed to increase the performance back.  
%    - new attacks to models that defended only one attacks
%    - new attacks to models that defended two attacks
%    - new attacks to models that defended three attacks
%\end{enumerate}

% \comGP{Are we making the same strong assumption from the FDA3 paper, that have an attack monitor capable of telling us which attack that we need to train against?}
% \comGP{I assume in this table for ii.) we will actually have ii.) how many epochs are needed to increase the performance back with adversarial training against the new attack (without randomisation); iii) same as ii.) but with adversarial training + randomisation?}
% \comZR{I assume we don't have the assumption of an attack monitor. This could be more practical. ii) yes. iii) yes, nice idea.}
% \comGP{> "I assume we don't have the assumption of an attack monitor. This could be more practical." 
% Don't we actually need to assume an attack monitor though? Or perhaps I misunderstood our adversarial training. I assumed that like in the FDA3 paper we tell each client which whitebox attack to train against. Perhaps we are just sampling uniformly across whitebox attacks and hoping for the best? (This strong assumption regarding the attack monitor is something that I don't like about this FDA3 paper by the way... had some initial ideas here how we could do something quite ambitious to help on this front. but defo not within the time remaining until the deadline ;-)...)}
% \comZR{I agree with you - don't like that as well. Our initial idea was to overthrow this assumption (and assume the original data is replaced by attack data). The adversarial training needs to know the attack scheme in FDA3 paper. We can only use the basic adversarial training idea - train real and fake data together. The performance may be bad (not sure yet). But this is why we use randomisation which does not need such a attack scheme monitor.}
% \comZR{'new attack' herein means the 4-th or even the 5-th attack schemes which the federated learning has not met before.}
% \comGP{>"'new attack' herein means the 4-th or even the 5-th attack schemes which the federated learning has not met before."
% Nice, ok, sold on this one. Therefore, a good finding would be if approaches using randomisation are more robust than the others for i.), and also bounce back faster for ii.). Cool.}
